Why Don't Developers Detect Improper Input Validation?'; DROP TABLE Papers; --

Improper Input Validation (IIV) is a software vulnerability that occurs when a system does not safely handle input data. Even though IIV is easy to detect and fix, it still commonly happens in practice. In this paper, we study to what extent developers can detect IIV and investigate underlying reasons. This knowledge is essential to better understand how to support developers in creating secure software systems. We conduct an online experiment with 146 participants, of which 105 report at least three years of professional software development experience. Our results show that the existence of a visible attack scenario facilitates the detection of IIV vulnerabilities and that a significant portion of developers who did not find the vulnerability initially could identify it when warned about its existence. Yet, a total of 60 participants could not detect the vulnerability even after the warning. Other factors, such as the frequency with which the participants perform code reviews, influence the detection of IIV. Data and materials: https://doi.org/10.5281/zenodo.3996696

==> sections/tab-variables.tex <==
%!TEX root=./security-developers.tex
\begin{table}
    \caption{Variables used in the logistic regression models.}\label{tab:vars}
    \centering
    \begin{tabular}{l|l}
    \hline
    \cellcolor[HTML]{C0C0C0}\textbf{Metric}             & \cellcolor[HTML]{C0C0C0}\textbf{Description} \\ \hline\hline
    \multicolumn{2}{c}{\cellcolor[HTML]{EFEFEF}\textit{Dependent Variables}}             \\ \hline
    \vf (\textbf{RQ$_{1}$})  & \begin{tabular}[c]{@{}l@{}}The participant found the vulnerability in the first \\ code review\end{tabular}               \\\hdashline[0.5pt/2pt]
    %\vnf & \begin{tabular}[c]{@{}l@{}}The participant did not find the vulnerability \\ during code review experiment \end{tabular}                                \\\hline
     \vfl (\textbf{RQ$_{2}$}) & \begin{tabular}[c]{@{}l@{}}The participant found the vulnerability during\\revisit to the code review        \end{tabular}                              \\\hline \hline
     
    \multicolumn{2}{c}{\cellcolor[HTML]{EFEFEF}\textit{Independent Variables}}             \\ \hline
    \vulntype                   & \begin{tabular}[c]{@{}l@{}} Type of the \iivShort vulnerability in the code change\\ (\sqliShort or \ivqiShort)\end{tabular}       \\\hline\hline  
    
    
    \multicolumn{2}{c}{\cellcolor[HTML]{EFEFEF}\textit{Control Variables   (Review)}}             \\ \hline
    \bug            & \begin{tabular}[c]{@{}l@{}}  The participant found the functional bug \end{tabular}       \\\hdashline[0.5pt/2pt]
    \inter               & \begin{tabular}[c]{@{}l@{}}For how long the participant was\\interrupted during the  review \end{tabular}      \\\hdashline[0.5pt/2pt]
    \reviewDuration                          & \begin{tabular}[c]{@{}l@{}}Duration of the code review\end{tabular}                                                           \\\hline
    \multicolumn{2}{c}{\cellcolor[HTML]{EFEFEF}\textit{Control Variables   (Security Knowledge)}}             \\ \hline
    \familiar                      & \begin{tabular}[c]{@{}l@{}} Familiarity to vulnerabilities\end{tabular} \\ \hdashline[0.5pt/2pt]
    \courses                      & \begin{tabular}[c]{@{}l@{}} The participant has participated in security \\ courses and/or training\end{tabular} \\ \hdashline[0.5pt/2pt]
    %%\training                     &\begin{tabular}[c]{@{}l@{}} The participant's security training is none/more\\ of the following: lecture, seminar, conference,\\hands-on courses, professional training \end{tabular}       \\\hdashline[0.5pt/2pt]
    %\lec                            & \begin{tabular}[c]{@{}l@{}} The participant attended lectures on  \\security \end{tabular}       \\\hdashline[0.5pt/2pt]
    %\conf                         & \begin{tabular}[c]{@{}l@{}}  The participant attended security  \\conferences\end{tabular}       \\\hdashline[0.5pt/2pt]
    %\sem                          & \begin{tabular}[c]{@{}l@{}}  The participant attended security  \\seminars\end{tabular}       \\\hdashline[0.5pt/2pt]
    %\handson                   & \begin{tabular}[c]{@{}l@{}}  The participant attended hands-on \\courses on security\end{tabular}       \\\hdashline[0.5pt/2pt]
   %\proftrain                   & \begin{tabular}[c]{@{}l@{}}  The participant attended professional\\training on security\end{tabular}       \\\hdashline[0.5pt/2pt]
    \update                      & \begin{tabular}[c]{@{}l@{}}  The participant keeps himself/herself up to date \\with security information \end{tabular}       \\\hline
    \multicolumn{2}{c}{\cellcolor[HTML]{EFEFEF}\textit{Control Variables   (Security Practice)}}             \\ \hline
    \incidents                   & \begin{tabular}[c]{@{}l@{}} The participant has experience with security \\incidents.\end{tabular}       \\\hdashline[0.5pt/2pt]
    \responsible            & \begin{tabular}[c]{@{}l@{}}  The participant looks for vulnerabilities as a\\part of his/her job responsibility \end{tabular}       \\\hdashline[0.5pt/2pt]
    %%\vulexp                       & \begin{tabular}[c]{@{}l@{}} The participant has experience in none or more \\of the following: vulnerability introduction,\\detection, fixing, exploitation.\end{tabular}       \\\hdashline[0.5pt/2pt]
    %\intvuln                       & \begin{tabular}[c]{@{}l@{}} The participant has ever introduced \\ a vulnerability or not during daily practice\end{tabular}       \\\hdashline[0.5pt/2pt]
    %\foundvuln                  & \begin{tabular}[c]{@{}l@{}} The participant has ever found \\ a vulnerability or not during daily practice\end{tabular}               \\\hdashline[0.5pt/2pt]
    %\fixvuln                       & \begin{tabular}[c]{@{}l@{}} The participant has ever fixed \\ a vulnerability or not during daily practice\end{tabular}                \\\hdashline[0.5pt/2pt]
    %\exploitvuln                & \begin{tabular}[c]{@{}l@{}} The participant has ever exploited \\ a vulnerability or not during daily practice\end{tabular}          \\\hdashline[0.5pt/2pt]
%    \practice                     & \begin{tabular}[c]{@{}l@{}} The participant uses in practice what (s)he has\\learnt about security\end{tabular}                        \\ \hdashline[0.5pt/2pt]
    \static                       & \begin{tabular}[c]{@{}l@{}}  How often the participant found static analysis\\tools helpful in finding vulnerabilities \end{tabular}       \\\hdashline[0.5pt/2pt]
    \dynamic                  & \begin{tabular}[c]{@{}l@{}}  How often the participant found dynamic analysis\\tools helpful in finding vulnerabilities \end{tabular}       \\\hdashline[0.5pt/2pt]
    \manual                    & \begin{tabular}[c]{@{}l@{}}  How often the participant found manual analysis\\helpful in finding vulnerabilities \end{tabular}       \\\hdashline[0.5pt/2pt]
    \design                   & \begin{tabular}[c]{@{}l@{}}  The participant actively considers vulnerabilities\\when designing software \end{tabular}       \\\hdashline[0.5pt/2pt]
    \code                      & \begin{tabular}[c]{@{}l@{}}  The participant actively considers vulnerabilities\\when coding \end{tabular}       \\\hdashline[0.5pt/2pt]
    \review                    & \begin{tabular}[c]{@{}l@{}}  The participant actively considers vulnerabilities\\when reviewing code \end{tabular}       \\\hline     
    
    \multicolumn{2}{c}{\cellcolor[HTML]{EFEFEF}\textit{Control Variables   (Team Culture)}}             \\ \hline
    %%\aware                    & \begin{tabular}[c]{@{}l@{}}  The extend to which developers in the team are\\aware of potential security issues\end{tabular}       \\\hdashline[0.5pt/2pt]
    %%\expert                   & \begin{tabular}[c]{@{}l@{}}  The extend to which developers in the team have \\security expertise \end{tabular}       \\\hdashline[0.5pt/2pt]
    \tools                     & \begin{tabular}[c]{@{}l@{}}  The extend to which developers in the team use\\tool to detect vulnerabilities \end{tabular}       \\\hdashline[0.5pt/2pt]
    \library                   & \begin{tabular}[c]{@{}l@{}}  The extend to which developers in  the team check\\for vulnerabilities in third party libraries\end{tabular}       \\\hdashline[0.5pt/2pt]
    \CRuse                        & \begin{tabular}[c]{@{}l@{}}  The extend to which developers in  the team use\\code review to detect vulnerabilities\end{tabular}       \\\hdashline[0.5pt/2pt]
    \timepressure       & \begin{tabular}[c]{@{}l@{}}  The extend to which developers in the team have\\time to consider security aspects\end{tabular}       \\\hline 
      \multicolumn{2}{c}{\cellcolor[HTML]{EFEFEF}\textit{Control Variables (demographics)}}             \\ \hline
    \gender                   & \begin{tabular}[c]{@{}l@{}}Gender of the participant\end{tabular}                                                          \\\hdashline[0.5pt/2pt]
    \loe                         & \begin{tabular}[c]{@{}l@{}}Highest achieved level of education\end{tabular}                                                          \\\hdashline[0.5pt/2pt]
    \emp                       & \begin{tabular}[c]{@{}l@{}}Employment status\end{tabular}                                                          \\\hdashline[0.5pt/2pt]
    \role                        & \begin{tabular}[c]{@{}l@{}}Role of the participant\end{tabular}                                                          \\\hdashline[0.5pt/2pt]
    %    \companysize          & \begin{tabular}[c]{@{}l@{}}Size of the company participant is working at\end{tabular}                                                          \\\hdashline[0.5pt/2pt]
    %    \teamsize                & \begin{tabular}[c]{@{}l@{}}Size of the participant's team\end{tabular}                                                          \\\hdashline[0.5pt/2pt]
    \oss                         & \begin{tabular}[c]{@{}l@{}}The participant's OSS development experience\end{tabular}                                                          \\\hdashline[0.5pt/2pt]
    \pde                         & \begin{tabular}[c]{@{}l@{}}Years of experience as professional \\developer\end{tabular}                                                          \\\hdashline[0.5pt/2pt]
    \je                          & \begin{tabular}[c]{@{}l@{}}Years of experience in Java\end{tabular}                                                          \\\hdashline[0.5pt/2pt]
    \rp                          & \begin{tabular}[c]{@{}l@{}}How often they perform code review\end{tabular}                                                          \\\hdashline[0.5pt/2pt]
    \re                          & \begin{tabular}[c]{@{}l@{}}Years of experience in code review\end{tabular}                                                          \\\hdashline[0.5pt/2pt]
    \web                       & \begin{tabular}[c]{@{}l@{}}Years of experience in web programming \end{tabular}                                                          \\\hdashline[0.5pt/2pt]
    \db                         & \begin{tabular}[c]{@{}l@{}}Years of experience in database applications \end{tabular}                                                          \\\hdashline[0.5pt/2pt]
    \designFreq            & \begin{tabular}[c]{@{}l@{}}How often they design software\end{tabular}                                                          \\\hdashline[0.5pt/2pt]
    \codingFreq            & \begin{tabular}[c]{@{}l@{}}How often they program\end{tabular}                                                          \\\hdashline[0.5pt/2pt]
    \crFreq                    & \begin{tabular}[c]{@{}l@{}}How often they review code\end{tabular}                                                          \\\hline
    
           

  
    %\multicolumn{2}{c}{\cellcolor[HTML]{EFEFEF}\textit{Control Variables}}             \\ \hline
    %\multicolumn{2}{c}{\cellcolor[HTML]{EFEFEF}\textit{Reviewer details}}             \\ \hline
    %\gender                   & \begin{tabular}[c]{@{}l@{}}Gender of the participant\end{tabular}                                                          \\\hdashline[0.5pt/2pt]
    %\loe                         & \begin{tabular}[c]{@{}l@{}}Highest achieved level of education\end{tabular}                                                          \\\hdashline[0.5pt/2pt]
    %\emp                       & \begin{tabular}[c]{@{}l@{}}Employment status\end{tabular}                                                          \\\hdashline[0.5pt/2pt]
    %\role                        & \begin{tabular}[c]{@{}l@{}}Role of the participant\end{tabular}                                                          \\\hdashline[0.5pt/2pt]
    %\companysize          & \begin{tabular}[c]{@{}l@{}}Size of the company participant is working at\end{tabular}                                                          \\\hdashline[0.5pt/2pt]
    %\teamsize                & \begin{tabular}[c]{@{}l@{}}Size of the participant's team\end{tabular}                                                          \\\hdashline[0.5pt/2pt]
    %\oss                         & \begin{tabular}[c]{@{}l@{}}The participant's Open Source Software (OSS) \\development experience\end{tabular}                                                          \\\hdashline[0.5pt/2pt]
    %\pde                         & \begin{tabular}[c]{@{}l@{}}Years of experience as professional \\developer\end{tabular}                                                          \\\hdashline[0.5pt/2pt]
    %\je                          & \begin{tabular}[c]{@{}l@{}}Years of experience in Java\end{tabular}                                                          \\\hdashline[0.5pt/2pt]
    %\rp                          & \begin{tabular}[c]{@{}l@{}}How often they perform code review\end{tabular}                                                          \\\hdashline[0.5pt/2pt]
    %\re                          & \begin{tabular}[c]{@{}l@{}}Years of experience in code review\end{tabular}                                                          \\\hdashline[0.5pt/2pt]
    %\web                       & \begin{tabular}[c]{@{}l@{}}Years of experience in web programming \end{tabular}                                                          \\\hdashline[0.5pt/2pt]
    %\db                         & \begin{tabular}[c]{@{}l@{}}Years of experience in database applications \end{tabular}                                                          \\\hdashline[0.5pt/2pt]
    %\designFreq            & \begin{tabular}[c]{@{}l@{}}How often they design software\end{tabular}                                                          \\\hdashline[0.5pt/2pt]
    %\codingFreq            & \begin{tabular}[c]{@{}l@{}}How often they program\end{tabular}                                                          \\\hdashline[0.5pt/2pt]
    %\crFreq                    & \begin{tabular}[c]{@{}l@{}}How often they review code\end{tabular}                                                          \\\hdashline[0.5pt/2pt]
    %\interfirst               & \begin{tabular}[c]{@{}l@{}}For how long the participant was\\interrupted during the code review  experiment\end{tabular}      \\\hdashline[0.5pt/2pt]
    %\intersecond          & \begin{tabular}[c]{@{}l@{}}For how long the participant was\\interrupted during revisit to the code review \end{tabular}      \\\hdashline[0.5pt/2pt]
    %\td                          & \begin{tabular}[c]{@{}l@{}}Total duration of the experiment\end{tabular}                                                          \\\hdashline[0.5pt/2pt]  \\\hline
   % \multicolumn{2}{r}{\emph{($\dagger$) see \Cref{fig:participants_details} for the scale}}             \\
    \end{tabular}
    \vspace{-1.5em}
    \end{table}

==> tabs/tab-rq2-oddsratio-comparing.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Sat Aug 29 10:30:12 2020
\begin{table}[ht]
\centering 
 \caption{Odds ratio for detecting the vulnerability in code review experiment and in the review revisit.} 
 \label{tab:rq2-oddsratio-comparing}
\begin{tabular}{lrrr}
 & \multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0}\textbf{Code Review}} & \multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0}\textbf{Revisit}} & \multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0}\textbf{}} \\ 
  \hline
SQL Injection & 52 & 13 \\ 
  Improper Valid. of Spec. Quantity Input & 14 & 7 \\ 
   \hline
\multicolumn{4}{r}{Odds Ratio: \oddsRatioComparing} \\ 
 \multicolumn{4}{r}{\bf\textit{p} \rhoComparing} \\ 
 \multicolumn{4}{r}{~} \\ 
 \end{tabular}
\end{table}


